Dustin: Draft-Augmented Sparse Verification for Efficient Long-Context Generation with Speculative Decoding

While speculative decoding improves inference throughput for multi-batch long-context Large Language Models (LLMs), its efficiency is often limited by a verification bottleneck where Key-Value (KV) cache loading dominates latency. Existing compression methods fail in this regime: static eviction incurs accuracy loss due to saliency shift, while dynamic selection introduces prohibitive computational overhead during the verification path. We propose Dustin, a sparse verification framework designed for long-context speculative decoding. Dustin integrates lookahead signals from the draft model with historical attention from the target model to identify critical tokens with high fidelity across multi-step verification windows. To reduce recomputation latency, this approach further employs a sparse estimation scheme that restricts importance scoring to a minimal subset of attention heads. Evaluations on PG-19 and LongBench with Qwen2.5-72B demonstrate that Dustin achieves a 27.85x speedup in self-attention and a 9.17x end-to-end decoding speedup at a 32k sequence length, all with negligible accuracy degradation.

==> latex/accuracy_table.tex <==
\begin{table*}[t]
  \caption{{\color{red}Accuracy evaluation on LongBench under two strict KV cache budgets (512 and 128 tokens). 
Quest follows its official setting where layers 0--1 do not apply KV compression, while SnapKV applies a one-time post-prefill prompt-KV compression and keeps the resulting prompt KV fixed during decode (no further prompt re-compression or eviction).}}
\centering
  \begin{adjustbox}{width=\textwidth}
  \begin{tabular}{l|c|c|c|c|c|c|c|c}
    \hline
    \textbf{Method} & \textbf{KV Size} & \textbf{Single-doc QA} & \textbf{Multi-doc QA} & \textbf{Summarization} & \textbf{Few-shot} & \textbf{Synthetic} & \textbf{Code} & \textbf{Avg.} \\
    \hline
    \multicolumn{9}{c}{\textit{Qwen2.5-72B-Instruct}} \\
    \hline
    FullKV           & ---                 & 44.23 & 57.00 & 27.54 & 72.55 & 60.00 & 66.70 & 55.81 \\
    \hline
    StreamingLLM     & \multirow{4}{*}{512}& 27.61 & 33.82 & 21.70 & 54.57 & 39.84 & 35.02 & 35.25 \\
    % SnapKV           &                     & 42.80 & \textbf{58.77} & 23.02 & 71.21 & 55.00 & 57.29 & 51.90 \\
    Quest*           &                     & 36.91 & 41.80 & 25.92 & 64.40 & 55.08 & 57.24 & 47.69 \\
    Dustin           &                     & \textbf{44.23} & 56.35 & \textbf{27.10} & \textbf{71.23} & \textbf{60.00} & \textbf{65.97} & \textbf{55.23} \\
    \hline
    StreamingLLM     & \multirow{4}{*}{128}& 23.27 & 32.49 & 17.58 & 48.48 & 42.69 & 33.68 & 32.72 \\
    % SnapKV           &                     & 36.57 & \textbf{56.89} & 19.80 & 63.71 & 51.63 & 51.54 & 47.08 \\
    Quest*           &                     & 23.12 & 25.21 & 21.67 & 52.81 & 49.70 & 46.37 & 37.01 \\
    Dustin           &                     & \textbf{44.59} & 55.31 & \textbf{26.14} & \textbf{68.35} & \textbf{52.13} & \textbf{61.30} & \textbf{52.41} \\
    \hline
    \multicolumn{9}{c}{\textit{Llama-3.3-70B-Instruct}} \\
    \hline
    FullKV           & ---                 & 45.48 & 58.88 & 28.58 & 70.75 & 53.63 & 49.64 & 50.94 \\
    \hline
    StreamingLLM     & \multirow{4}{*}{512}& 32.36 & 39.35 & 23.01 & 51.55 & 51.05 & 41.98 & 39.61 \\
    % SnapKV           &                     & 44.45 & \textbf{59.58} & 24.87 & 68.75 & 53.39 & 58.82 & 52.41 \\
    Quest*            &                     & 40.34 & 52.24 & 27.18 & 66.63 & \textbf{54.61} & 51.95 & 48.96 \\
    Dustin           &                     & \textbf{45.27} & 59.10 & \textbf{27.76} & \textbf{70.14} & 53.40 & \textbf{59.15} & \textbf{53.23} \\
    \hline
    StreamingLLM     & \multirow{4}{*}{128}& 27.13 & 39.78 & 19.02 & 46.43 & 52.44 & 39.49 & 36.94 \\
    % SnapKV           &                     & 39.17 & 58.02 & 22.07 & 64.55 & \textbf{54.63} & 58.53 & 50.32 \\
    Quest*            &                     & 23.66 & 27.93 & 21.09 & 47.94 & 44.20 & 35.67 & 33.21 \\
    Dustin           &                     & \textbf{45.55} & \textbf{59.02} & \textbf{26.75} & \textbf{68.18} & 53.96 & \textbf{62.78} & \textbf{53.81} \\
    \hline
  \end{tabular}
  \end{adjustbox}
  \label{tab:acc_results}
\end{table*}
